The Keck-HGCA Pilot Survey II: Direct Imaging Discovery of HD 63754 B, a ~20 au Massive Companion Near the Hydrogen Burning Limit

We present the joint astrometric and direct imaging discovery, mass measurement, and orbital analysis of HD 63754 B (HIP 38216 B), a companion near the stellar-substellar boundary orbiting ~20 AU from its Sun-like host. HD 63754 was observed in our ongoing high-contrast imaging survey targeting stars with significant proper-motion accelerations between Hipparcos and Gaia consistent with wide-separation substellar companions. We utilized archival HIRES and HARPS radial velocity (RV) data, together with the host star's astrometric acceleration extracted from the Hipparcos-Gaia Catalog of Accelerations (HGCA), to predict the location of the candidate companion around HD 63754 A. We subsequently imaged HD 63754 B at its predicted location using the Near Infrared Camera 2 (NIRC2) in the $L'$ band at the W. M. Keck Observatory. We then jointly modeled the orbit of HD 63754 B with RVs, Hipparcos-Gaia accelerations, and our new relative astrometry, measuring a dynamical mass of ${81.9}_{-5.8}^{+6.4} M_{jup}$, an eccentricity of ${0.260}_{-0.059}^{+0.065}$, and a nearly face-on inclination of $174.81_{-0.50}^{+0.48}$ degrees. For HD 63754 B, we obtain an L' band absolute magnitude of $L' = 11.39\pm0.06$ mag, from which we infer a bolometric luminosity of $log(L_{bol}/L_{\odot})= -4.55 \pm0.08$ dex using a comparison sample of L and T dwarfs with measured luminosities. Although uncertainties linger in age and dynamical mass estimates, our analysis points toward HD 63754 B's identity as a brown dwarf on the L/T transition rather than a low-mass star, indicated by its inferred bolometric luminosity and model-estimated effective temperature. Future RV, spectroscopic, and astrometric data such as those from JWST and Gaia DR4 will clarify HD 63754 B's mass, and enable spectral typing and atmospheric characterization.

==> hgca_accel_mnras.tex <==


\begin{table*}
\centering
\caption{HGCA absolute astrometry for HD~176535~A.}
\label{table:hgca_absAst}
\begin{tabular}{lccc}
	    \hline
Parameter & Hipparcos & Hipparcos-Gaia & Gaia EDR3 \\
\hline
% hipid: 93398 rv: -31.704752 gaiaplx: 27.032526 chisq: 8208.919
% $\mu_{\alpha, Hip}$    &-21.855$\pm$1.344\\
% $\mu_{\delta, Hip}$    &-32.098$\pm$0.996\\
% $corr_{Hip}$     &0.130\\
% $t_{\alpha,Hip}$     &1991.27\\
% $t_{\delta,Hip}$    &1991.41\\
% $\mu_{\alpha, HG}$    &-22.016$\pm$0.048\\
% $\mu_{\delta, HG}$    &-32.295$\pm$0.030\\
% $corr_{HG}$     &-0.024\\
% $\mu_{\alpha, Gaia}$    &-24.927$\pm$0.025\\
% $\mu_{\delta, Gaia}$    &-29.707$\pm$0.022\\
% $corr_{Gaia}$     &0.214\\
% $t_{\alpha,Gaia}$     &2016.27\\
% $t_{\delta,Gaia}$    &2016.36\\
% $\chi^{2}$  &8208.919\\ 
$\mu_{\alpha*}$ (mas\,yr$^{-1}$)   &$-21.9 \pm 1.3$ & $-22.016 \pm 0.048$ & $-24.927 \pm 0.025$\\
 $\mu_{\delta}$ (mas\,yr$^{-1}$)&$ -32.1 \pm 1.0$ & $-32.295 \pm 0.030$ & $-29.707 \pm 0.022 $\\
 ${\rm corr}(\mu_{\alpha*},\mu_{\delta})$     &0.13 & $-0.02$ & $0.21$ \\
 $t_{\alpha}$ (Jyr)    &1991.27 & & 2016.27 \\
 $t_{\delta}$ (Jyr)    &1991.41 & & 2016.36 \\\hline
% $\chi^{2}$  &8208.919\\
\end{tabular} \\
{\sc Note:} The $\chi^2$ value for a model of constant proper motion (Hipparcos-Gaia \\ and Gaia proper motions are equal) is 8215 with two degrees of freedom.
\end{table*}
